Multiplex graph matching matched filters

We consider the problem of detecting a noisy induced multiplex template network in a larger multiplex background network. Our approach, which extends the framework of Sussman et al. (2019) to the multiplex setting, leverages a multiplex analogue of the classical graph matching problem to use the template as a matched filter for efficiently searching the background for candidate template matches. The effectiveness of our approach is demonstrated both theoretically and empirically, with particular attention paid to the potential benefits of considering multiple channels.

==> deleted_bibs.tex <==
@article{foggia2014graph,
  title={Graph matching and learning in pattern recognition in the last 10 years},
  author={Foggia, P. and Percannella, G. and Vento, M.},
  journal={International Journal of Pattern Recognition and Artificial Intelligence},
  volume={28},
  number={01},
  pages={1450001},
  year={2014},
  publisher={World Scientific}
}
% @article{graphhomobased,
%   title={Faster algorithms for finding and counting subgraphs},
%   author={Fomin, F. V. and Lokshtanov, D. and Raman, V. and Saurabh, S. and Rao, B. V. R.},
%   journal={Journal of Computer and System Sciences},
%   volume={78},
%   number={3},
%   pages={698--706},
%   year={2012},
%   publisher={Elsevier}
% }

% @inproceedings{sgsurvey,
%   title={An in-depth comparison of subgraph isomorphism algorithms in graph databases},
%   author={Lee, J. and Han, W. and Kasperovics, R. and Lee, J.},
%   booktitle={Proceedings of the VLDB Endowment},
%   volume={6},
%   number={2},
%   pages={133--144},
%   year={2012},
%   organization={VLDB Endowment}
% }
% @article{efficienttreesearch,
%   title={An algorithm for subgraph isomorphism},
%   author={Ullmann, J. R.},
%   journal={Journal of the ACM (JACM)},
%   volume={23},
%   number={1},
%   pages={31--42},
%   year={1976},
%   publisher={ACM}
% }
% @inproceedings{yan2016short,
%   title={A short survey of recent advances in graph matching},
%   author={Yan, J. and Yin, X. and Lin, W. and Deng, C. and Zha, H. and Yang, X.},
%   booktitle={Proceedings of the 2016 ACM on International Conference on Multimedia Retrieval},
%   pages={167--174},
%   year={2016},
%   organization={ACM}
% }
% @article{foggia2014graph,
%   title={Graph matching and learning in pattern recognition in the last 10 years},
%   author={Foggia, P. and Percannella, G. and Vento, M.},
%   journal={International Journal of Pattern Recognition and Artificial Intelligence},
%   volume={28},
%   number={01},
%   pages={1450001},
%   year={2014},
%   publisher={World Scientific}
% }

% @inproceedings{takes2017detecting,
%   title={Detecting Motifs in Multiplex Corporate Networks},
%   author={Takes, F. W. and Kosters, W. A. and Witte, B.},
%   booktitle={International Workshop on Complex Networks and their Applications},
%   pages={502--515},
%   year={2017},
%   organization={Springer}
% }
% @incollection{yang2016mining,
%   title={Mining Multiplex Structural Patterns from Complex Networks},
%   author={Yang, B. and Liu, J.},
%   booktitle={Wisdom Web of Things},
%   pages={275--301},
%   year={2016},
%   publisher={Springer}
% }
% @article{feasibilityrules,
%   title={A (sub) graph isomorphism algorithm for matching large graphs},
%   author={Cordella, L. P. and Foggia, P. and Sansone, C. and Vento, M.},
%   journal={IEEE Transactions on Pattern Analysis and Machine Intelligence},
%   volume={26},
%   number={10},
%   pages={1367--1372},
%   year={2004},
%   publisher={IEEE}
% }
% @article{colorcoding1,
%   title={Color-coding},
%   author={Alon, N. and Yuster, R. and Zwick, U.},
%   journal={Journal of the ACM (JACM)},
%   volume={42},
%   number={4},
%   pages={844--856},
%   year={1995},
%   publisher={ACM}
% }
% @article{colorcoding2,
%   title={Biomolecular network motif counting and discovery by color coding},
%   author={Alon, N. and Dao, P. and Hajirasouliha, I. and Hormozdiari, F. and Sahinalp, S. C.},
%   journal={Bioinformatics},
%   volume={24},
%   number={13},
%   pages={i241--i249},
%   year={2008},
%   publisher={Oxford University Press}
% }

% @article{foggia2014graph,
%   title={Graph matching and learning in pattern recognition in the last 10 years},
%   author={Foggia, P. and Percannella, G. and Vento, M.},
%   journal={International Journal of Pattern Recognition and Artificial Intelligence},
%   volume={28},
%   number={01},
%   pages={1450001},
%   year={2014},
%   publisher={World Scientific}
%   }
% @article{jointLi,
%   title={A joint graph inference case study: {T}he {C}. elegans chemical and electrical connectomes},
%   author={Chen, L. and Vogelstein, J. T. and Lyzinski, V. and Priebe, C. E.},
%   journal={Worm},
%   volume={5},
%   number={2},
%   year={2016},
%   organization={Taylor \& Francis}
% }
% @article{ConteReview,
% author = {Conte, D. and Foggia, P. and Sansone, C. and Vento, M.},
% title = {Thirty years of graph matching in pattern recognition},
% journal = {International Journal of Pattern Recognition and Artificial Intelligence},
% volume = {18},
% number = {03},
% pages = {265-298},
% year = {2004},
% }


% @article{mucha2010community,
%   title={Community structure in time-dependent, multiscale, and multiplex networks},
%   author={Mucha, P. J. and Richardson, T. and Macon, K. and Porter, M. A. and Onnela, J.},
%   journal={Science},
%   volume={328},
%   number={5980},
%   pages={876--878},
%   year={2010},
%   publisher={American Association for the Advancement of Science}
% }
